Contaminated Online Convex Optimization

In online convex optimization, some efficient algorithms have been designed for each of the individual classes of objective functions, e.g., convex, strongly convex, and exp-concave. However, existing regret analyses, including those of universal algorithms, are limited to cases in which the objective functions in all rounds belong to the same class and cannot be applied to cases in which the property of objective functions may change in each time step. This paper introduces a novel approach to address such cases, proposing a new regime we term as \textit{contaminated} online convex optimization. For the contaminated case, we demonstrate that the regret is lower bounded by $\Omega(\log T + \sqrt{k})$. Here, $k$ signifies the level of contamination in the objective functions. We also demonstrate that the regret is bounded by $O(\log T+\sqrt{k\log T})$ when universal algorithms are used. When our proposed algorithms with additional information are employed, the regret is bounded by $O(\log T+\sqrt{k})$, which matches the lower bound. These are intermediate bounds between a convex case and a strongly convex or exp-concave case.

==> 6_proposed.tex <==
\section{Regret Upper Bounds Given Additional Information}\label{sec:proposed}

In this section, we propose two methods that achieve better bounds than those of universal algorithms discussed in the previous section, under the condition that parameters $k$, $\alpha$, and $\lambda$ are known and the information of the class of the last objective function is revealed.
One is for $k$-contaminated exp-concave case and the other is for $k$-contaminated strongly convex case.
The experimental performances of these proposed methods are shown in Appendix~\ref{sec:exp}.

\subsection{$k$-Contaminated Exp-Concave Case}

Let $(f_1,f_2,\ldots,f_T)$ be $k$-contaminated $\alpha$-exp-concave.
We denote $S\coloneqq\{t\in[T]\mid f_t~\mathrm{is}~\alpha\text{-exp-concave}\}$ and $U\coloneqq[T]\backslash S$.
By this definition, $|U|=k$ holds.
Using this notation, we set parameters $\gamma_t$ as follows:
\[\gamma_t=
\begin{dcases}
  \gamma&t\in S,\\
  0&t\in U.
\end{dcases}
\]

Proposed method is shown in Algorithm~\ref{alg:con-ons} ($\|\cdot\|_{\bm A}^2$ means $\pro{\bm A\cdot}{\cdot}$).
This algorithm is a generalization of ONS and we call it contaminated ONS.
Indeed, setting $k=0$ gives normal ONS.
The setting of parameters $\gamma_t$ reflects contamination.

\begin{algorithm}[tb]
    \caption{Contaminated ONS}
    \begin{algorithmic}[1]\label{alg:con-ons}    
    \REQUIRE convex set $\mathcal X\subset\R^d$, $\bm x_1\in\mathcal X$, $T$, $k$, $D$, $G$, $\alpha$
    \STATE Set $\gamma\coloneqq(1/2)\min\{1/(GD),\alpha\}$, $\varepsilon\coloneqq(G/D)\sqrt k$, $\bm A_0\coloneqq\varepsilon \bm I_d$.
    \FOR{$t=1$ {\bfseries to} $T$}
    \STATE Play $\bm x_t$ and observe cost $f_t(\bm x_t)$.
    \STATE Set $\gamma_t=\gamma~(t\in S),~0~(t\in U)$. 
    \STATE Rank-1 update: 
    \[
      \bm A_t=\bm A_{t-1}+\gamma_t\nabla f_t(\bm x_t)(\nabla f_t(\bm x_t))^\top.
    \]
    \STATE Newton step and generalized projection:
    \[
      \bm y_{t+1}=\bm x_t-\bm A_t^{-1}\nabla f_t(\bm x_t),
    \]
    \[
      \bm x_{t+1}=\Pi_{\mathcal X}^{\bm A_t}(\bm y_{t+1})\coloneqq\argmin_{\bm x\in\mathcal X}\{\|\bm y_{t+1}-\bm x\|_{\bm A_t}^2\}.
    \]
    \ENDFOR
    \end{algorithmic}
\end{algorithm}

The following theorem bounds the regret of contaminated ONS:

\begin{theorem}\label{thm:con-ons}
    If $(f_1,f_2,\ldots,f_T)$ is $k$-contaminated $\alpha$-exp-concave, Algorithm~\ref{alg:con-ons} guarantees 
    \[
        R_T=O\left(\frac d\gamma\log T+GD\sqrt k\right).
    \]
\end{theorem}

\begin{proof}
Let $\bm x^\ast\in\argmin_{\bm x\in\mathcal X}\sum_{t=1}^Tf_t(\bm x)$.
From Lemma~\ref{ecineq}, we have
\begin{align*}
  2(f_t(\bm x_t)-f_t(\bm x^\ast))
  &\leq2\pro{\nabla f_t(\bm x_t)}{\bm x_t-\bm x^\ast}-\gamma_t(\pro{\nabla f_t(\bm x_t)}{\bm x_t-\bm x^\ast})^2\\
  &=2\pro{\bm A_t(\bm y_{t+1}-\bm x_t)}{\bm x^\ast-\bm x_t}-\|\bm x_t-\bm x^\ast\|_{\bm A_{t}}^2+\|\bm x_t-\bm x^\ast\|_{\bm A_{t-1}}^2\\
  &=\|\bm y_{t+1}-\bm x_t\|_{\bm A_t}^2-\|\bm y_{t+1}-\bm x^\ast\|_{\bm A_t}^2+\|\bm x_t-\bm x^\ast\|_{\bm A_{t-1}}^2\\
  &\leq\|\bm y_{t+1}-\bm x_t\|_{\bm A_t}^2-\|\bm x_{t+1}-\bm x^\ast\|_{\bm A_t}^2+\|\bm x_t-\bm x^\ast\|_{\bm A_{t-1}}^2.
\end{align*}
The first equality is from the algorithm, the second equality is from the low of cosines, and the last inequality is from the nonexpansiveness of projection.
By summing up from $t=1$ to $T$, we can bound regret as follows:
\begin{align*}
  2R_T
  &\leq\sum_{t=1}^T\|\bm y_{t+1}-\bm x_t\|_{\bm A_t}^2+\|\bm x_1-\bm x^\ast\|_{\bm A_{0}}^2\\
  &\leq\sum_{t=1}^T\|\nabla f_t(\bm x_t)\|_{\bm A_t^{-1}}^2+D^2\varepsilon\\
  &=\sum_{t\in S}\|\nabla f_t(\bm x_t)\|_{\bm A_t^{-1}}^2+\sum_{t\in U}\|\nabla f_t(\bm x_t)\|_{\bm A_t^{-1}}^2+D^2\varepsilon.
\end{align*}

% For the first term, we can bound as follows:
% \begin{align}
%   \sum_{t\in S}\|\nabla f_t(\bm x_t)\|_{\bm A_t^{-1}}^2
%   &\leq\frac d\gamma\log\frac{\varepsilon+\gamma G^2T}{\varepsilon}.\label{eq:first_term}
% \end{align}
% The derivation of this inequality is postponed to Appendix~???, since its main idea is the same as the analysis for normal ONS by~\citet{hazan16}.

% The inequality is from Lemma~\ref{lem:for_ons} in Appendix~\ref{sec:for_ons}, the third equality is from $\bm A_t=\bm A_{t-1}~(\forall t\in U)$, and the last is from the fact that the largest eigenvalue of $\bm A_T$ is at most $\varepsilon+\gamma G^2T$.



For the first term, we can bound as follows:
\begin{align*}
  \sum_{t\in S}\|\nabla f_t(\bm x_t)\|_{\bm A_t^{-1}}^2
  &=\sum_{t\in S}\tr(\bm A_t^{-1}\nabla f_t(\bm x_t)(\nabla f_t(\bm x_t))^\top)\\
  &=\frac1\gamma\sum_{t\in S}\tr(\bm A_t^{-1}(\bm A_t-\bm A_{t-1}))\\
  &\leq\frac1\gamma\sum_{t\in S}\log\frac{|\bm A_t|}{|\bm A_{t-1}|}\\
  &=\frac1\gamma\log\frac{|\bm A_T|}{|\bm A_{0}|}\\
  &=\frac d\gamma\log\frac{\varepsilon+\gamma G^2T}{\varepsilon}.
\end{align*}
The inequality is from Lemma~\ref{lem:for_ons} in Appendix~\ref{sec:for_ons}, the third equality is from $\bm A_t=\bm A_{t-1}~(\forall t\in U)$, and the last is from the fact that the largest eigenvalue of $\bm A_T$ is at most $\varepsilon+\gamma G^2T$.



For the second term, we can bound as follows:
\[
  \sum_{t\in U}\|\nabla f_t(\bm x_t)\|_{\bm A_t^{-1}}^2
  \leq \sum_{t\in U}\frac{G^2}\varepsilon\\
  = \frac{G^2k}\varepsilon.
\]

Therefore, by taking $\varepsilon\coloneqq(G/D)\sqrt k$, we can get
\begin{align*}
  2R_T
  &\leq\frac d\gamma\log\frac{\varepsilon+\gamma G^2T}{\varepsilon}+\frac{G^2k}\varepsilon+D^2\varepsilon\\
  &=\frac d\gamma\log(1+\gamma GD\frac T{\sqrt k})+2GD\sqrt k\\
  &=O\left(\frac d\gamma\log T+GD\sqrt k\right).
\end{align*}
\end{proof}

The key point of Theorem~\ref{thm:con-ons} is that the second term of the regret upper bound is proportional to $\sqrt k$.
Comparing with Corollary~\ref{ecmetagradmalerusc}, we can see that additional information improves the regret upper bound.



\subsection{$k$-Contaminated Strongly Convex Case}\label{sec:con-ogd}

Let $(f_1,f_2,\ldots,f_T)$ be $k$-contaminated $\lambda$-strongly convex and $f_t$ be $\lambda_t$-strongly convex ($\lambda_t=0$ is possible).
By \citet{hazan2007adaptive}, it is already known that if OGD (Algorithm~\ref{alg:ogd} in Appendix~\ref{ogdalg}) is performed on the regularized functions $\tilde f_t(\bm x)\coloneqq f_t(\bm x)+(\mu_t/2)\|\bm x\|^2$ with stepsizes
\begin{align}
    \eta_t\coloneqq\left(\sum_{s=1}^t(\lambda_s+\mu_s)\right)^{-1},\label{stepsize}
\end{align}
then 
\begin{align}
    R_T\leq\frac{D^2}2\sum_{t=1}^T\mu_t+\sum_{t=1}^T\eta_t(\mu_t^2D^2+G^2),\label{reg-ogd}
\end{align}
where $R_T$ is the regret not for $\tilde f_t$ but for $f_t$.
Using this bound, we can get the following bound for the contaminated case.

\begin{theorem}\label{thm:con-ogd}
    If $(f_1,f_2,\ldots,f_T)$ is $k$-contaminated $\lambda$-strongly convex, OGD on the regularized functions $\tilde f_t$ with stepsizes defined in equation~\ref{stepsize} and 
    $\mu_1=\sqrt k$, $\mu_t=0$ $(1<t\leq T)$
    guarantees
    \[
        R_T=O\left(\frac{G^2}\lambda\log T+(D^2+G^2)\sqrt k\right).
    \]
\end{theorem}

\begin{proof}
    Let $\tilde k_t$ be the integer such that $(f_1,f_2,\ldots,f_t)$ is $\tilde k_t$-contaminated $\lambda$-strongly convex.
    By the definition, $\tilde k_t$ satisfies
    $\tilde k_t\leq\min\{k,t\}$.
    From this inequality and inequality~\ref{reg-ogd}, we can bound the regret as follows:
    \begin{align*}
    R_T
    &\leq\frac{D^2}2\sqrt k+\frac{kD^2}{\lambda_1+\sqrt k}+\sum_{t=1}^T\frac{G^2}{(t-\tilde k_t)\lambda+\sqrt k}\\
    &\leq\frac32D^2\sqrt k+\sum_{t=1}^{k}\frac{G^2}{\sqrt k}+\sum_{t=k+1}^{T}\frac{G^2}{(t-k)\lambda+\sqrt k}\\
    &\leq\left(\frac32D^2+G^2\right)\sqrt k+\int_{k}^{T}\frac{G^2}{(t-k)\lambda+\sqrt k}\dd t\\
    &=\left(\frac32D^2+G^2\right)\sqrt k+\frac{G^2}\lambda\log\left(\frac \lambda{\sqrt k}(T-k)+1\right)\\
    &=O\left(\frac{G^2}\lambda\log T+(D^2+G^2)\sqrt k\right).
    \end{align*}
\end{proof}

The key point of Theorem~\ref{thm:con-ogd} is the same as mentioned to Theorem~\ref{thm:con-ons}; the second term is proportional to $\sqrt k$.
Comparing with Corollary~\ref{scmetagradmalerusc}, we can see the improvement.



\color{blue}
\begin{remark}\label{rem:hybrid}
    We can consider the hybrid algorithm of Algorithm~\ref{alg:con-ons} and the algorithm explained in subsection~\ref{sec:con-ogd} by utilizing the idea of Follow The Approximate Leader (FTAL)~\citep{hazan06}.
    Since the algorithm of the hybrid version and its regret analysis is almost same as what has been explained in this section, details are postponed to Appendix~\ref{sec:hybrid}.
\end{remark}
\color{black}



\begin{remark}
    As mentioned in Remark~\ref{rem:prior}, the algorithms analyzed in this section need some information which is not always available in real world.
    Therefore, the improved regret bounds in Theorem~\ref{thm:con-ons} and Theorem~\ref{thm:con-ogd} are theoretical ones, and regret bounds for universal algorithms explained in Section~\ref{upperbounds} are more important in real application.
    However, the regret analyses in this section are insightful because the existence of the upper bound with additional $O(\sqrt k)$ term implies that the regret upper bounds of universal algorithms in Section~\ref{upperbounds} can be improved.
\end{remark}



% \subsection{{\color{blue}Variant of Maler}}
% The algorithm is based on the idea of Maler~\citep{wang20}.
% We denote $S_1\coloneqq\{t\in[T]\mid f_t~\mathrm{is}~\lambda\text{-strongly convex}\}$, $S_2\coloneqq\{t\in[T]\mid f_t~\mathrm{is}~\alpha\text{-exp-concave}\}$, and $U\coloneqq[T]\backslash (S_1\cup S_2)$.
% Let 
% \begin{align*}
%     s_t^\eta(\bm x)&\coloneqq-\eta\pro{\nabla f_t(\bm x_t)}{\bm x_t-\bm x}+\eta^2G^2\|\bm x_t-\bm x\|^2,\\
%     \ell_t^\eta(\bm x)&\coloneqq-\eta\pro{\nabla f_t(\bm x_t)}{\bm x_t-\bm x}+\eta^2(\pro{\nabla f_t(\bm x_t)}{\bm x_t-\bm x})^2,\\
%     c_t(\bm x)&\coloneqq-\eta^c\pro{\nabla f_t(\bm x_t)}{\bm x_t-\bm x}+(\eta^cGD)^2.
% \end{align*}
% Since $\e^{x-x^2}\leq1+x$ for any {\color{blue}$x\geq-2/3$}~\citep{erven16}, we have
% \begin{align*}
%     \e^{-s_t^\eta(\bm x_t^{\eta,s})}&\leq1+\eta\pro{\nabla f_t(\bm x_t)}{\bm x_t-\bm x_t^{\eta,s}},\\
%     \e^{-\ell_t^\eta(\bm x_t^{\eta,\ell})}&\leq1+\eta\pro{\nabla f_t(\bm x_t)}{\bm x_t-\bm x_t^{\eta,\ell}},\\
%     \e^{-c_t(\bm x_t^{\eta,c})}&\leq1+\eta^c\pro{\nabla f_t(\bm x_t)}{\bm x_t-\bm x_t^{c}},
% \end{align*}
% for each $\eta$.

% Define a potential function
% \[
%     \Phi_t=
%     \sum_\eta(\pi_1^{\eta,s}\e^{-\sum_{\tau\in S_1\cap[t]}s_\tau^\eta(\bm x_\tau^{\eta,s})}
%     +\pi_1^{\eta,\ell}\e^{-\sum_{\tau\in S_2\cap[t]}\ell_\tau^\eta(\bm x_\tau^{\eta,\ell})})
%     +\pi_1^c\e^{-\sum_{\tau\in U\cap[t]}c_\tau(\bm x_\tau^c)}.
% \]
% If $t+1\in S_1$,
% \begin{align*}
%     \Phi_{t+1}-\Phi_t
%     &=\sum_\eta\pi_1^{\eta,s}\e^{-\sum_{\tau\in S_1\cap[t]}s_\tau^\eta(\bm x_\tau^{\eta,s})}(\e^{-s_{t+1}^\eta(\bm x_{t+1}^{\eta,s})}-1)\\
%     &\leq\sum_\eta\pi_1^{\eta,s}\e^{-\sum_{\tau\in S_1\cap[t]}s_\tau^\eta(\bm x_\tau^{\eta,s})}\eta\pro{\nabla f_{t+1}(\bm x_{t+1})}{\bm x_{t+1}-\bm x_{t+1}^{\eta,s}},
% \end{align*}
% if $t+1\in S_2$,
% \begin{align*}
%     \Phi_{t+1}-\Phi_t
%     &=\sum_\eta\pi_1^{\eta,\ell}\e^{-\sum_{\tau\in S_2\cap[t]}\ell_\tau^\eta(\bm x_\tau^{\eta,\ell})}(\e^{-\ell_{t+1}^\eta(\bm x_{t+1}^{\eta,\ell})}-1)\\
%     &\leq\sum_\eta\pi_1^{\eta,\ell}\e^{-\sum_{\tau\in S_2\cap[t]}\ell_\tau^\eta(\bm x_\tau^{\eta,\ell})}\eta\pro{\nabla f_{t+1}(\bm x_{t+1})}{\bm x_{t+1}-\bm x_{t+1}^{\eta,\ell}},
% \end{align*}
% and if $t+1\in U$,
% \begin{align*}
%     \Phi_{t+1}-\Phi_t
%     &=\sum_\eta\pi_1^{\eta,s}\e^{-\sum_{\tau\in U\cap[t]}s_\tau^\eta(\bm x_\tau^{\eta,s})}(\e^{-s_{t+1}^\eta(\bm x_{t+1}^{\eta,s})}-1)\\
%     &\leq\sum_\eta\pi_1^{\eta,s}\e^{-\sum_{\tau\in U\cap[t]}s_\tau^\eta(\bm x_\tau^{\eta,s})}\eta\pro{\nabla f_{t+1}(\bm x_{t+1})}{\bm x_{t+1}-\bm x_{t+1}^{\eta,s}}.
% \end{align*}

% To guarantee that $\Phi_t$ is non-increasing, we take
% \begin{align*}
%     \bm x_{t+1}=\begin{dcases}
%         \frac{\sum_\eta\pi_{t+1}^{\eta,s}\eta\bm x_{t+1}^{\eta,s}}{\sum_\eta\pi_{t+1}^{\eta,s}\eta},&{\color{blue}t+1\in S_1}
%     \end{dcases}
% \end{align*}
% where
% \begin{align*}
%     \pi_{t+1}^{\eta,s}=\pi_1^{\eta,s}\prod_{\tau=1}^t\frac{\e^{-1_{S_1}(\tau)s_\tau^\eta(\bm x_\tau^{\eta,s})}}{\Phi_\tau}
% \end{align*}

% {\color{blue}To realize this algorithm, we have to use the information at time step $t+1\ldots$}




% \begin{algorithm}[tb]
%     \caption{Variant of Maler}
%     \label{alg:malervariant}
%     \begin{algorithmic}[1]
%     \REQUIRE $T$, $G$, $D$, $C=1+1/(1+\lceil(1/2)\log_2T\rceil)$
%     \STATE Set  {\color{blue}$\eta^c=1/(2GD\sqrt T)$}, $\eta_i=2^{-i}/(5GD)$.
%     \STATE Set $\pi^c=1/3,~\pi_1^{\eta_i,\ell}=\pi_1^{\eta_i,s}= C/(3(i+1)(i+2))$ for $i=0,1,\ldots,\lceil(1/2)\log_2T\rceil$.
%     % \STATE Set $\Phi_0=1$.
%     \FOR{$t=1$ {\bfseries to} $T$}
%     \STATE {\color{blue}Play $\bm x_t=\frac{\pi_t^c\eta^c\bm x_t^c+\sum_\eta(\pi_t^{\eta,s}\eta\bm x_t^{\eta,s}+\pi_t^{\eta,\ell}\eta\bm x_t^{\eta,\ell})}{\pi_t^c\eta^c+\sum_\eta(\pi_t^{\eta,s}\eta+\pi_t^{\eta,\ell}\eta)}$ and observe cost $f_t(\bm x_t)$.}
%     \STATE Update weights:
%     \[
%     \pi_{t+1}^c=\frac{\pi_t^c\e^{-c_t(\bm x_t^c)}}{\Phi_t},
%     \]
%     \[
%     \pi_{t+1}^{\eta,s}=\frac{\pi_t^{\eta,s}\e^{-s_t^\eta(\bm x_t^{\eta,s})}}{\Phi_t}~\text{for~all}~\eta,
%     \]
%     \[
%     \pi_{t+1}^{\eta,\ell}=\frac{\pi_t^{\eta,\ell}\e^{-\ell_t^\eta(\bm x_t^{\eta,\ell})}}{\Phi_t}~\text{for~all}~\eta,
%     \]
%     where
%     \[
%     \Phi_t=\sum_\eta(\pi_1^{\eta,s}\e^{-\sum_{\tau\in S_1\cap[t]}s_\tau^\eta(\bm x_\tau^{\eta,s})}+\pi_1^{\eta,\ell}\e^{-\sum_{\tau\in S_2\cap[t]}\ell_\tau^\eta(\bm x_\tau^{\eta,\ell})})+\pi_1^c\e^{-\sum_{\tau\in U\cap[t]}c_\tau(\bm x_\tau^c)}.
%     \]
%     \IF{$f_t$ is $\lambda$-strongly convex}
%     \STATE Update for all $\eta$:
%     \[
%     \bm x_{t+1}^{\eta,s}=\Pi_{\mathcal X}\left(\bm x_t^{\eta,s}-\frac1{2\eta^2G^2t}\nabla s_t^\eta(\bm x_t^{\eta,s})\right).
%     \]
%     \ELSIF{$f_t$ is $\alpha$-exp-concave}
%     \STATE Update for all $\eta$:
%     \[
%     \bm \Sigma_{t+1}=\bm\Sigma_t+\nabla\ell_t^\eta(\bm x_t^{\eta,\ell})(\nabla\ell_t^\eta(\bm x_t^{\eta,\ell}))^\top,
%     \]
%     \[
%     \bm x_{t+1}^{\eta,\ell}=\Pi_{\mathcal X}^{\bm\Sigma_{t+1}}\left(\bm x_t^{\eta,\ell}-\frac1\beta\bm\Sigma_{t+1}^{-1}\nabla \ell_t^\eta(\bm x_t^{\eta,\ell})\right).
%     \]
%     \ELSE
%     \STATE Update:
%     \[
%     \bm x_{t+1}^c=\Pi_{\mathcal X}\left(\bm x_t^c-\frac D{\eta^cG\sqrt t}\nabla c_t(\bm x_t^c)\right).
%     \]
%     \ENDIF
%     \ENDFOR
%     \end{algorithmic}
% \end{algorithm}













% \subsection{{\color{blue}Algorithm}}
% The algorithm is based on the idea of FTAL~\citep{hazan06}.
% We denote $S_1\coloneqq\{t\in[T]\mid f_t~\mathrm{is}~\alpha\text{-exp-concave}\}$, $S_2\coloneqq\{t\in[T]\mid f_t~\mathrm{is}~\lambda\text{-strongly convex}\}$, and $U\coloneqq[T]\backslash (S_1\cup S_2)$.
% For each round $t\in[T]$, we consider the following subproblem:
% \begin{align*}
%     \argmin_{\bm x\in\mathcal X}\sum_{\tau=1}^{t}\bar f_\tau(\bm x)+\frac\varepsilon2\|\bm x\|^2,
% \end{align*}
% where
% \begin{align*}
%     \bar f_t(\bm x)\coloneqq\begin{dcases}
%         \pro{\nabla f_t(\bm x_t)}{\bm x-\bm x_t}+\frac\gamma2(\pro{\nabla f_t(\bm x_t)}{\bm x-\bm x_t})^2,&t\in S_1,\\
%         \pro{\nabla f_t(\bm x_t)}{\bm x-\bm x_t}+\frac\lambda2\|\bm x-\bm x_t\|^2,&t\in S_2,\\
%         \pro{\nabla f_t(\bm x_t)}{\bm x-\bm x_t},&t\in U.
%     \end{dcases}
% \end{align*}

% The subproblem mentioned above is equivalent to the following optimization problem:
% \begin{align}
%     \argmin_{\bm x\in\mathcal X}\frac12\|\bm x\|_{\bm A_{t}}^2-\pro{\bm b_{t}}{\bm x},\label{prob:hybrid}
% \end{align}
% where 
% \begin{align*}
%     \bm A_0&=\varepsilon\bm I_n,~\bm A_t=\bm A_{t-1}+\begin{dcases}
%         \gamma\nabla f_t(\bm x_t)\nabla f_t(\bm x_t)^\top,&t\in S_1\\
%         \lambda\bm I_n,&t\in S_2\\
%         \bm O_n,&t\in U,
%     \end{dcases}\\
%     \bm b_0&=\bm 0,~\bm b_t=\bm b_{t-1}-\begin{dcases}
%         \nabla f_t(\bm x_t)-\gamma\pro{\nabla f_t(\bm x_t)}{\bm x_t}\nabla f_t(\bm x_t),&t\in S_1,\\
%         \nabla f_t(\bm x_t)-\lambda\bm x_t,&t\in S_2,\\
%         \nabla f_t(\bm x_t),&t\in U.\\
%     \end{dcases}
% \end{align*}

% The solution of the optimization problem~\ref{prob:hybrid} is $\Pi_{\mathcal X}^{\bm A_{t}}(\bm A_{t}^{-1}\bm b_{t})$ by the definition of the projection.

% This procedure gives the hybrid algorithm shown in Algorithm~\ref{alg:hybrid2}.



% \begin{algorithm}[tb]
%     \caption{{\color{blue}Hybrid Algorithm???}}
%     \begin{algorithmic}[1]\label{alg:hybrid2}    
%     \REQUIRE convex set $\mathcal X\subset\R^d$, $\bm x_1\in\mathcal X$, $T$, $k$, $D$, $G$, $\alpha$
%     \STATE Set $\gamma\coloneqq(1/2)\min\{1/(GD),\alpha\}$, $\varepsilon\coloneqq(G/D)\sqrt k$, $\bm A_0\coloneqq\varepsilon \bm I_d$, $\bm b_0=\bm 0$.
%     \FOR{$t=1$ {\bfseries to} $T$}
%     \STATE Play $\bm x_t$ and observe cost $f_t(\bm x_t)$.
%     \STATE Update: 
%     \[
%       \bm A_t=\bm A_{t-1}+\begin{dcases}
%         \gamma\nabla f_t(\bm x_t)\nabla f_t(\bm x_t)^\top,&t\in S_1\\
%         \lambda\bm I_d,&t\in S_2\\
%         \bm O_d,&t\in U,
%     \end{dcases}
%     \]
%     \[
%         \bm b_t=\bm b_{t-1}-\begin{dcases}
%         \nabla f_t(\bm x_t)-\gamma\pro{\nabla f_t(\bm x_t)}{\bm x_t}\nabla f_t(\bm x_t),&t\in S_1,\\
%         \nabla f_t(\bm x_t)-\lambda\bm x_t,&t\in S_2,\\
%         \nabla f_t(\bm x_t),&t\in U.
%         \end{dcases}
%     \]
%     \STATE Generalized projection:
%     \[
%       \bm y_{t+1}=\bm A_t^{-1}\bm b_t,
%     \]
%     \[
%       \bm x_{t+1}=\Pi_{\mathcal X}^{\bm A_t}(\bm y_{t+1}).
%     \]
%     \ENDFOR
%     \end{algorithmic}
% \end{algorithm}



% \subsection{{\color{blue}Regret Upper Bound of Hybrid Algorithm}}
